WaveAttack: Asymmetric Frequency Obfuscation-based Backdoor Attacks Against Deep Neural Networks

Due to the popularity of Artificial Intelligence (AI) technology, numerous backdoor attacks are designed by adversaries to mislead deep neural network predictions by manipulating training samples and training processes. Although backdoor attacks are effective in various real scenarios, they still suffer from the problems of both low fidelity of poisoned samples and non-negligible transfer in latent space, which make them easily detectable by existing backdoor detection algorithms. To overcome the weakness, this paper proposes a novel frequency-based backdoor attack method named WaveAttack, which obtains image high-frequency features through Discrete Wavelet Transform (DWT) to generate backdoor triggers. Furthermore, we introduce an asymmetric frequency obfuscation method, which can add an adaptive residual in the training and inference stage to improve the impact of triggers and further enhance the effectiveness of WaveAttack. Comprehensive experimental results show that WaveAttack not only achieves higher stealthiness and effectiveness, but also outperforms state-of-the-art (SOTA) backdoor attack methods in the fidelity of images by up to 28.27\% improvement in PSNR, 1.61\% improvement in SSIM, and 70.59\% reduction in IS.

==> broaderImpact.tex <==
\section{Broader Impact and Limitations}\label{limitation}
\textbf{Broader Impact.} In this work, we introduce a new effective and stealthy backdoor attack method named WaveAttack, which can stealthily compromise security-critical systems. If used improperly, the proposed attack method may pose a security risk to the existing DNN applications. Nevertheless, we hope that by emphasizing the potential harm of this malicious threat model, our work will stimulate the development of stronger defenses and promote greater attention from experts in the field. As a result, this knowledge will promote the creation of more secure and dependable DNN models and robust defensive measures.

\textbf{Limitations.} Our approach WaveAttack requires more computing resources and runtime overhead than most existing backdoor attack methods, due to the necessity of training a generator $g$ to generate residuals of the high-frequency component. Moreover, we do not consider a more standard threat model, in which the adversary can only control the training dataset. In this threat model, we used our pre-trained generator to modify some benign samples in the training dataset. Our approach WaveAttack has limited effectiveness. This limitation also appears in Qi et al. \cite{backdoorat-adapt}. In the future, we will explore more effective and stealthy backdoor attack methods in this threat model. 
